SubRegWeigh: Effective and Efficient Annotation Weighing with Subword Regularization

NLP datasets may still contain annotation errors, even when they are manually annotated. Researchers have attempted to develop methods to automatically reduce the adverse effect of errors in datasets. However, existing methods are time-consuming because they require many trained models to detect errors. This paper proposes a time-saving method that utilizes a tokenization technique called subword regularization to simulate multiple error detection models for detecting errors. Our proposed method, SubRegWeigh, can perform annotation weighting four to five times faster than the existing method. Additionally, SubRegWeigh improved performance in document classification and named entity recognition tasks. In experiments with pseudo-incorrect labels, SubRegWeigh clearly identifies pseudo-incorrect labels as annotation errors. Our code is available at https://github.com/4ldk/SubRegWeigh .

==> latex/tables/case_study.tex <==

\begin{table*}[!h]
\begin{tabular}{llrrrr}
\hline \hline
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{CrossWeigh} & \multicolumn{3}{c}{SubRegWeigh} \\
\multicolumn{1}{c}{Text} & \multicolumn{1}{c}{Label} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Random} & \multicolumn{1}{c}{Cos-Sim} & \multicolumn{1}{c}{$K$-means} \\ \hline
\begin{tabular}[c]{@{}l@{}}The foreign ministry ’s Shen \\ told Reuters Television in an\\  interview he had read reports \\ of Tang ’s comments ...\end{tabular} & \begin{tabular}[c]{@{}l@{}}O O O O \underline{B-ORG} \\ O B-ORG I-ORG \\ O O O O O O O \\ O B-PER O O ...\end{tabular} & 0.343 & 0.333 & 0.333 & 0.333 \\ \hline
\begin{tabular}[c]{@{}l@{}}NOTES BAYERISCHE \\ VEREINSBANK IS \\ JOINT LEAD MANAGER\end{tabular} & \begin{tabular}[c]{@{}l@{}}O B-ORG I-ORG\\ O O O O\end{tabular} & 0.7 & 0.5 & 0.5 & 0.333 \\ \hline
\begin{tabular}[c]{@{}l@{}}Former Surinam rebel \\ leader held after shooting .\end{tabular} & \begin{tabular}[c]{@{}l@{}}O \underline{B-LOC O} O \\ O O O O\end{tabular} & 1.0 & 0.7 & 0.7 & 0.5 \\ \hline \hline
\end{tabular}
\caption{Case study. Underlined are incorrect or ambiguous labels.CW means weights generated by CrossWeigh, SRW means weights generated by SubRegWeigh.}
\label{tab:case_study}
\end{table*}

